Stabilizing Consensus is Impossible in Lossy Iterated Immediate Snapshot Models

A substantial portion of distributed computing research is dedicated to terminating problems like consensus and similar agreement problems. However, non-terminating problems have been intensively studied in the context of self-stabilizing distributed algorithms, where processes may start from arbitrary initial states and can tolerate arbitrary transient faults. In between lie stabilizing problems, where the processes start from a well-defined initial state, but do not need to decide irrevocably and are allowed to change their decision finitely often until a stable decision is eventually reached. In this paper, we introduce the novel Delayed Lossy-Link (DLL) model, and the Lossy Iterated Immediate Snapshot Model (LIIS), for which we show stabilizing consensus to be impossible. The DLL model is introduced as a variant of the well-known Lossy-Link model, which admits silence periods of arbitrary but finite length. The LIIS model is a variant of the Iterated Immediate Snapshot (IIS), model which admits finite length periods of at most $f$ omission faults per layer. In particular, we show that stabilizing consensus is impossible even when $f=1$. Our results show that even in a model with very strong connectivity, namely, the Iterated Immediate Snapshot (IIS) model, a single omission fault per layer effectively disables stabilizing consensus. Furthermore, since the DLL model always has a perpetual broadcaster, the mere existence of a perpetual broadcaster, even in a crash-free setting, is not sufficient for solving stabilizing consensus, negatively answering the open question posed by Charron-Bost and Moran.

==> comment_responses.tex <==
Dear Petr,

thank you for reaching out. We have taken the liberty of indexing the comments below and addressing each of the 5 points individually. We clear the major concern (2) as the mentioned related work critically assumes a different adversarial model and thus is not admissible in our case.

(1) Seeing failure detectors as stabilizing tasks: 

We are aware of the connection between stabilizing tasks and failure detectors, as well as the work on terminating task solvability with respect to systems with failure detectors such as [24] where Raynal and Stainer equated various asynchronous systems with failure detectors to synchronous message adversaries. However they do not explicitly state the failure detectors as a stabilizing task $T_{FD}$, and even in that case, the solvability of $T_{FD}$ as a stabilizing task would be connected to the terminating task solvability of another task $T$. In contrast, we lift the solvability of a stabilizing task $T$ in a model M to a terminating instance of the exact same task $T$ in a different model $M'$. We would be very happy to include these considerations and elaborate further within the related works and conclusion.

(2) Asymptotic consensus in the DLL: [FNS21] and [8] assume oblivious message adversaries. The DLL is NOT an oblivious message adversary, and for this reason the results in neither [FNS21] nor [8] are applicable to the DLL. 

Furthermore the following averaging algorithm solves asymptotic consensus in the DLL, code for process p:
x = input
T(Msgs):
    if (q, x_q) in Msgs:
        x = (x+x_q)/2
S():
    return (p, x).

It should be noted that asymptotic consensus allows processes to decide from a continuous pool of values, while stabilizing agreement only allows for decisions within the set of input values. In this sense, asymptotic consensus is closer to stabilizing approximate agreement than to stabilizing agreement. As it is mentioned in the comments, stabilizing consensus implies asymptotic consensus, but not necessarily the other way around. In general, asymptotic consensus is weaker.

(3) 2 process vs. n-processes: as in the celebrated FLP impossibility result, proving that stabilizing agreement is impossible for two processes (under certain circumstances, i.e., unbound silent rounds) transparently translates to n processes. More concretely, the 3-process case is explicitly extended to a model with $n$ processes in Corollary 5.2. Furthermore, we claim that stabilizing agreement can also be trivially shown impossible in a model where the DLL or the BAMP(n,f) is embeddable as a submodel via a simple simulation that extends on the proof of Corollary 5.2.
We would be happy to elaborate on this in the final version.

(4) MinMax in Section 3: Theorem 3.2 shows that the Lossy Link Message Adversary has a rootedness of 1, showing that it has a non-empty kernel and a bounded diameter, i.e., the MinMax correctly runs on a LL Message Adversary. This, together with Section 3.1., re-proves (in order to be self-contained) the parts from [9] needed in this paper.
We acknowledge that Section 3 would profit from a concise and explicit theorem summing up the results from Section 3 in accordance with its description in the introduction. We would be happy to accommodate for it in the final version.

(5) MinMax in the DLL: The MinMax algorithm is unable to solve stabilizing agreement in the DLL. Moreover, due to page limit concerns, we had to drop the depiction of the MinMax algorithm in the LL model and an exemplary failing execution in DLL model, but we would be very happy to include it in a final version.

Best regards,
Hugo, Stephan

===

(1) Regarding related works, it is claimed this is the first time terminating computability and stabilizing computability are shown to be equivalent on some models. Since, as it is mentionned in the conclusion, failure detectors can be seen as stabilizing tasks, and that there are a full body of work investigating how to convert such stabilizing tasks into terminating ones, there should be more nuance there.

(2) More important in my opinion is the fact that asymptotic consensus is overlooked. It is mentionned but not discussed. Asymptotic consensus is the task where processes have to agree only in the limit. It is straightforward to see that stabilizing consensus implies asymptotic consensus. Therefore any impossibility proof for asymptotic consensus gives an impossibility proof for stabilizing consensus. From [6], and [8] and [FNS21] it seems pretty clear that asymptotic consensus should not be solvable in DLL. If this is not that straightforward, this should be at least argumented and discussed.

[FNS21] Függer M, Nowak T, Schwarz M. Tight Bounds for Asymptotic and Approximate Consensus. J ACM. 28 oct 2021;68(6):46:1-46:35.

(3) Another difficulty is following the exposition and the results. This is only deep inside the paper that the reader will realize that the claimed results in the introduction are only for two processes. While investigating a distributed system of only two processes is not a default per se, it is important to stress since the introduction the actual scope of the results. It is also unclear how, if applicable, those results for two processes can be extended to any process. 

(4) There also formal flaws in the presentation like indicating in the outline that there is a result about using MinMax to solve the task at hand in section 3, without any corresponding theorems there (it seems they are deferred, without mentionning it, to the Appendix).

(5) Regarding the MinMax algorithm, it seems really strange that there is no explicit depiction of this algorithm for only two processes (ie binary consensus), since it is such a simplified instance in DLL : only solo runs with input value 1 stabilize to 1 if I understand correctly.

=== 

==> leftovers.tex <==
\iffalse
\subsection{The \emph{Iterated Immediate Snapshot Model} and the \emph{Lossy-Link Model}}
\label{subsec:IISLL}

The \emph{Iterated Immediate Snapshot} (abbreviated as IIS) model is an asynchronous shared
memory model, where processes communicate through snapshots. A snapshot consists of an
instantaneous write-read operation in which a process writes into an assigned register, and proceeds
to read the complete memory at once. The snapshot operation is concurrent, and multiple
processes can execute the snapshot operation at the same time, implying that for two
processes $\p$ and $\q$, there are only 3 possible outcomes for a single round:
either $\p$ executed its snapshot first, or $\q$ executed the snapshot
first, or $\p$ and $\q$ execute their snapshots concurrently.

Although a snapshot operation is not practical, it has been shown to hold the exact same
computability power as asynchronous single-read single-write wait-free shared memory
models~\cite{BG93}, thus making the snapshot model convenient for computability analysis.
Furthermore the IIS Model allows us to relate task solvability in asynchronous shared memory
to spatial properties via combinatorial topology, as shown in~\cite{HS94}. In turn the
combinatorial topology approach has yielded results such as the $k$-set agreement
impossibility for asynchronous shared memory.

Interestingly enough, in the case of 2 processes ($\Pi = \{ \p, \q \}$), the
IIS Model is equivalent to the Lossy-Link model. In the Lossy-Link model we
consider a synchronous message passing system where any communication graph
sequence is allowed, as long as it does not include the empty graph, i.e., at
any round some process is able to communicate to the other. Both in the IIS and
in synchronous message passing we have one possible global initial state given
the process \p and \q's initial state together they form the only one possible
initial configuration. In \cref{fig:iis_initial_config} \tp, \tq represent \p and
\q's initial state respectively, the edge connecting them represents the only
legal composition of the two states which is also the only initial configuration.

\begin{figure}[ht]
  \label{fig:iis_initial_config}
  \begin{tikzpicture}
  \pgfmathsetmacro{\xstart}{0}
  \pgfmathsetmacro{\xlength}{12}
  \pgfmathsetmacro{\ystart}{0}
  \pgfmathsetmacro{\ystep}{2}

    \pgfmathtruncatemacro{\ty}{\ystart+(\ystep)*2}
    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*0}
    \node[ps,label={}] at (\tx, \ty) (\ty0) {};

    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*9}
    \node[qs,label={}] at (\tx, \ty) (\ty1) {};

    \draw[] (\ty0) -- (\ty1);
  \end{tikzpicture}
  \caption{The initial configuration of a 2 processor Iterated Immediate Snapshot
  model, assuming the initial states of \tp and \tq are given.}
\end{figure}

In the first round of the IIS model the information processes receive depends
on when (with respect to each other) they start the snapshot operation. We have
three different possibilities: \p writes then reads the whole memory before \q
writes anything, resulting in \p not learning anything new, or vice versa. Lastly
\p and \q can write and read concurrently resulting in both reading each others
messages. For both \p and \q one round of communication results in two possible states
(i.e., in total four states), namely the state where they did not hear anything (they
were too fast) and the state where they read the other process' message.

As with the initial states, we connect legal combinations of local states with
an edge, representing a possible global configuration, i.e., a valid step of the
system. In \cref{fig:iis_one_round} the three possible communication patterns are
the three edges. \tp on the left has to be the state where \p did not read \q's 
message, because it is adjacent to just one possible communication pattern and
we only have one communication pattern where \p does not learn anything, similar
for \tq on the right. The two states, \tq and \tp, in the middle thus both read
each others message and their connecting edge in the center represents the third
possible communication pattern, the concurrent snapshots.

\begin{figure}[ht]
  \label{fig:iis_one_round}
  \begin{tikzpicture}
  \pgfmathsetmacro{\xstart}{0}
  \pgfmathsetmacro{\xlength}{12}
  \pgfmathsetmacro{\ystart}{0}
  \pgfmathsetmacro{\ystep}{1}

    \pgfmathtruncatemacro{\ty}{\ystart+(\ystep)*2}
    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*0}
    \node[ps,label={}] at (\tx, \ty) (\ty0) {};

    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*9}
    \node[qs,label={}] at (\tx, \ty) (\ty1) {};

    \draw[] (\ty0) -- (\ty1);
    
    % ---
    
    \pgfmathtruncatemacro{\ty}{\ystart+(\ystep)*1}
    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*0}
    \node[ps] at (\tx, \ty) (\ty0) {};
    
        \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*3}
        \node[qs,label={}] at (\tx, \ty) (\ty1) {};
        
        \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*6}
        \node[ps,label={}] at (\tx, \ty) (\ty2) {};

    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*9}
    \node[qs] at (\tx, \ty) (\ty3) {};

    %\draw[] (\ty0) -- (\ty1) -- (\ty2) -- (\ty3);
    \draw[-{Latex[length=2mm]}] (\ty0) -- (\ty1) ;
    \draw[{Latex[length=2mm]}-{Latex[length=2mm]}] (\ty1) -- (\ty2) ;
    \draw[-{Latex[length=2mm]}] (\ty3) -- (\ty2) ;

    \pgfmathtruncatemacro{\tty} {\ystart+(\ystep)*1}
    \pgfmathtruncatemacro{\ttty}{\ystart+(\ystep)*2}
    \draw[dotted,->] (\ttty0) -- (\tty0);
    \draw[dotted,->] (\ttty1) -- (\tty3);
  \end{tikzpicture}
  \caption{The possible configurations after one round of the lossy-link system.
  The edge in the middle represents \tp and \tq heard from each other, the edges
  on the left and right represent that \tq heard from \tp and \tp from \tq respectively.
  The arrowheads indicate "which messages arrived", however they should purely build
  intuition and have no formal meaning.}
\end{figure}

Notice that this construction of all possible configurations after one round of
communication was completely independent of the current round (in this case, round $1$).
Intuitively we just divided the edge (i.e., the only possible initial configuration) by
two states and thus already constructed all possible developments of that configuration
in one round of communication.
We can inductively apply this construction on each of the resulting possible configurations,
further advancing the system to any desired depth. \cref{fig:iis_second_round} depicts the
IIS model after two rounds of communication.

% We can now evaluate this model after one round of communication, where both
% processes first write to their respective cells and then read the other cell.
% As already mentioned above, the only impossible case is where both processes read $\bot$
% in the other process' cell. The possible system states after one round of
% communication can be pictured as in \cref{fig:iis_one_round}: either $\q$ read
% what $\p$ wrote (and $\p$ reads $\bot$, represented by the edge on the left), both
% read what the other process wrote (represented by the edge in the middle), or $\p$
% read what $\q$ wrote (and $\q$ reads $\bot$, represented by the edge on the right).


\begin{figure}[ht]
  \begin{tikzpicture}
  \pgfmathsetmacro{\pangle}{20}
  \pgfmathsetmacro{\qangle}{-20}
  \pgfmathsetmacro{\xstart}{0}
  \pgfmathsetmacro{\xlength}{12}
  \pgfmathsetmacro{\ystart}{0}
  \pgfmathsetmacro{\ystep}{1}

    \pgfmathtruncatemacro{\ty}{\ystart+(\ystep)*2}
    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*0}
    \node[ps,label={}] at (\tx, \ty) (\ty0) {};

    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*9}
    \node[qs,label={}] at (\tx, \ty) (\ty1) {};

    \draw[] (\ty0) -- (\ty1);
    
    % ---
    
    \pgfmathtruncatemacro{\ty}{\ystart+(\ystep)*1}
    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*0}
    \node[ps] at (\tx, \ty) (\ty0) {};
    
        \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*3}
        \node[qs,label={}] at (\tx, \ty) (\ty1) {};
        
        \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*6}
        \node[ps,label={}] at (\tx, \ty) (\ty2) {};

    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*9}
    \node[qs] at (\tx, \ty) (\ty3) {};

    %\draw[] (\ty0) -- (\ty1) -- (\ty2) -- (\ty3);
    \draw[-{Latex[length=2mm]}] (\ty0) -- (\ty1) ;
    \draw[{Latex[length=2mm]}-{Latex[length=2mm]}] (\ty1) -- (\ty2) ;
    \draw[-{Latex[length=2mm]}] (\ty3) -- (\ty2) ;
    
    % ---

    \pgfmathtruncatemacro{\ty}{\ystart+(\ystep)*0}
    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*0}
    \node[ps] at (\tx, \ty) (\ty0) {};
    
            \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*1}
            \node[qs,label={}] at (\tx, \ty) (\ty1) {};
            \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*2}
            \node[ps,label={}] at (\tx, \ty) (\ty2) {};
    
        \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*3}
        \node[qs] at (\tx, \ty) (\ty3) {};
        
            \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*4}
            \node[ps,label={}] at (\tx, \ty) (\ty4) {};
            \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*5}
            \node[qs,label={}] at (\tx, \ty) (\ty5) {};
        
        \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*6}
        \node[ps] at (\tx, \ty) (\ty6) {};
        
            \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*7}
            \node[qs,label={}] at (\tx, \ty) (\ty7) {};
            \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*8}
            \node[ps,label={}] at (\tx, \ty) (\ty8) {};

    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*9}
    \node[qs] at (\tx, \ty0) (\ty9) {};

    %\draw[] (\ty0) -- (\ty1) -- (\ty2) -- (\ty3) -- (\ty4) -- (\ty5) -- (\ty6) -- (\ty7) -- (\ty8) -- (\ty9);
    \draw[-{latex[length=2mm]}] (\ty0) -- (\ty1) ;
    \draw[{latex[length=2mm]}-{latex[length=2mm]}] (\ty1) -- (\ty2) ;
    \draw[-{latex[length=2mm]}] (\ty3) -- (\ty2) ;
    \draw[-{latex[length=2mm]}] (\ty3) -- (\ty4) ;
    \draw[{latex[length=2mm]}-{latex[length=2mm]}] (\ty4) -- (\ty5) ;
    \draw[-{latex[length=2mm]}] (\ty6) -- (\ty5) ;
    \draw[-{latex[length=2mm]}] (\ty6) -- (\ty7) ;
    \draw[{latex[length=2mm]}-{latex[length=2mm]}] (\ty7) -- (\ty8) ;
    \draw[-{latex[length=2mm]}] (\ty9) -- (\ty8) ;

    \pgfmathtruncatemacro{\ty}  {\ystart+(\ystep)*0}
    \pgfmathtruncatemacro{\tty} {\ystart+(\ystep)*1}
    \pgfmathtruncatemacro{\ttty}{\ystart+(\ystep)*2}
    \draw[dotted,->] (\ttty0) -- (\tty0);
    \draw[dotted,->] (\tty0) -- (\ty0);
   
    \draw[dotted,->] (\ttty1) -- (\tty3);
    \draw[dotted,->] (\tty3) -- (\ty9);
    
    \draw[dotted,->] (\tty1) -- (\ty3);
    \draw[dotted,->] (\tty2) -- (\ty6);
    
  \end{tikzpicture}
  \caption{The possible IIS configurations after two rounds of communication. We
  can see that already nine possible global states are allowed after just two rounds
  of exchanging information.}
  \label{fig:iis_second_round}
\end{figure}
\fi

\iffalse
\begin{figure}[ht]
  \label{fig:dll_second_round}
  \begin{tikzpicture}[state/.style={circle,draw}]
  \pgfmathsetmacro{\pangle}{20}
  \pgfmathsetmacro{\qangle}{-20}
  \pgfmathsetmacro{\xstart}{0}
  \pgfmathsetmacro{\xlength}{12}
  \pgfmathsetmacro{\ystart}{0}
  \pgfmathsetmacro{\ystep}{2}

    \pgfmathtruncatemacro{\ty}{\ystart+(\ystep)*2}
    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*0}
    \node[ps,label={$p$}] at (\tx, \ty) (\ty0) {};

    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*9}
    \node[qs={80},label={$q$}] at (\tx, \ty) (\ty1) {};

    \draw[] (\ty0) -- (\ty1);
    
    % ---
    
    \pgfmathtruncatemacro{\ty}{\ystart+(\ystep)*1}
    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*0}
    \node[ps] at (\tx, \ty) (\ty0) {};
    
        \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*3}
        \node[qs] at (\tx, \ty) (\ty1) {};
        
        \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*6}
        \node[ps] at (\tx, \ty) (\ty2) {};

    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*9}
    \node[qs] at (\tx, \ty) (\ty3) {};
    \draw[-{Latex[length=3mm]}] (\ty0) -- (\ty1) ;
    \draw[{Latex[length=3mm]}-{Latex[length=3mm]}] (\ty1) -- (\ty2) ;
    \draw[-{Latex[length=3mm]}] (\ty3) -- (\ty2) ;
    \draw [] (\ty0) to[out=340,in=200] (\ty3);
    
    % ---

    \pgfmathtruncatemacro{\ty}{\ystart+(\ystep)*0}
    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*0}
    \node[ps] at (\tx, \ty) (\ty0) {};
    
            \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*1}
            \node[qs] at (\tx, \ty) (\ty1) {};
            \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*2}
            \node[ps] at (\tx, \ty) (\ty2) {};
    
        \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*3}
        \node[qs] at (\tx, \ty) (\ty3) {};
        \node[qs] at (\tx, \ty-1) (\ty10) {};
        \draw[-{Latex[length=2mm]}] (\ty0) to[out=340,in=170] (\ty10) ;
        
            \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*4}
            \node[ps] at (\tx, \ty) (\ty4) {};
            \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*5}
            \node[qs] at (\tx, \ty) (\ty5) {};
        
        \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*6}
        \node[ps] at (\tx, \ty) (\ty6) {};
        \node[ps] at (\tx, \ty-1) (\ty11) {};
        \draw[{Latex[length=2mm]}-{Latex[length=2mm]}] (\ty10) to[out=350,in=190](\ty11) ;
        
            \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*7}
            \node[qs] at (\tx, \ty) (\ty7) {};
            \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*8}
            \node[ps] at (\tx, \ty) (\ty8) {};

    \pgfmathsetmacro{\tx}{\xstart+(\xlength/10)*9}
    \node[qs] at (\tx, \ty0) (\ty9) {};
    
    \draw[-{Latex[length=2mm]}] (\ty9) to[out=200,in=10] (\ty11) ;
    
    \draw[-{latex[length=2mm]}] (\ty0) -- (\ty1) ;
    \draw[{latex[length=2mm]}-{latex[length=2mm]}] (\ty1) -- (\ty2) ;
    \draw[-{latex[length=2mm]}] (\ty3) -- (\ty2) ;
    \draw[-{latex[length=2mm]}] (\ty3) -- (\ty4) ;
    \draw[{latex[length=2mm]}-{latex[length=2mm]}] (\ty4) -- (\ty5) ;
    \draw[-{latex[length=2mm]}] (\ty6) -- (\ty5) ;
    \draw[-{latex[length=2mm]}] (\ty6) -- (\ty7) ;
    \draw[{latex[length=2mm]}-{latex[length=2mm]}] (\ty7) -- (\ty8) ;
    \draw[-{latex[length=2mm]}] (\ty9) -- (\ty8) ;
    \draw [] (\ty0) to[out=20,in=160] (\ty3);
    \draw [] (\ty3) to[out=20,in=160] (\ty6);
    \draw [] (\ty6) to[out=20,in=160] (\ty9);
    \draw [] (\ty0) to[out=320,in=220] (\ty9);

    \pgfmathtruncatemacro{\ty}  {\ystart+(\ystep)*0}
    \pgfmathtruncatemacro{\tty} {\ystart+(\ystep)*1}
    \pgfmathtruncatemacro{\ttty}{\ystart+(\ystep)*2}
    \draw[dotted,->] (\ttty0) -- (\tty0);
    \draw[dotted,->] (\tty0) -- (\ty0);
   
    \draw[dotted,->] (\ttty1) -- (\tty3);
    \draw[dotted,->] (\tty3) -- (\ty9);
    
    \draw[dotted,->] (\tty1) -- (\ty3);
    \draw[dotted,->] (\tty2) -- (\ty6);
    
  \end{tikzpicture}
  \caption{2-round Delayed Lossy-Link.}
\end{figure}
\fi


\iffalse
\begin{wrapfigure}{l}{0.35\textwidth}
\vspace{-10pt}
\begin{tikzpicture}

    \node at (0, 0) (r1) {$\delta_p(\sigma : \none : \none^k)$};
    \node at (0, 1) (r2) {$\delta_p(\sigma : \pq : \none^k)$};
    \node at (0, 2) (r3) {$\delta_q(\sigma : \pq : \none^k)$};
    \node at (0, 3) (r4) {$\delta_q(\sigma : \pqp : \none^k)$};
    \node at (0, 4) (r5) {$\delta_p(\sigma : \pqp : \none^k)$};
    \node at (0, 5) (r6) {$\delta_p(\sigma : \qp : \none^k)$};
    \node at (0, 6) (r7) {$\delta_q(\sigma : \qp : \none^k)$};
    \node at (0, 7) (r8) {$\delta_q(\sigma : \none : \none^k)$};

    \foreach \i in {1, 3, 5, 7} {
        \pgfmathtruncatemacro{\j}{\i+1}
        \draw (r\i.west) .. controls +(left:0.4cm) and +(left:0.4cm) .. (r\j.west)
            node[midway,draw,circle,inner sep=2pt,fill=white] {$=$};
    }

    \foreach \i in {2, 4, 6} {
        \pgfmathtruncatemacro{\j}{\i+1}
        \draw (r\i.east) .. controls +(right:0.4cm) and +(right:0.4cm) .. (r\j.east)
            node[midway,draw,circle,inner sep=2pt,fill=white] {$?$};
    }

    \draw (r1.east) .. controls +(right:2cm) and +(right:2cm) .. (r8.east)
        node[midway,draw,circle,inner sep=2pt,fill=white] {$\neq$};
\end{tikzpicture}
\caption{ dsalkjf }
\label{fig:forever_undecided_run}
\vspace{-5pt}
\end{wrapfigure}
\fi


\iffalse
\begin{figure}[ht]
  \label{fig:dll_one_round}
  \begin{tikzpicture}
    \node[ps,label=:{$T(p_1^0, \bot)$}] at (0, 0) (p10) {$p_1^1$};

    \node[qs={60},label=:{$T(p_1^0, p_2^0)$}] at (2, 0) (q11) {$p_2^1$};
    \node[ps={60},label=:{$T(p_1^0, p_2^0)$}] at (4, 0) (p11) {$p_1^1$};

    \node[qs,label=:{$T(\bot, p_2^0)$}] at (6, 0) (q10) {$p_2^1$};

    \draw[-{Latex[length=3mm]}] (p10) -- (q11) ;
    \draw[{Latex[length=3mm]}-{Latex[length=3mm]}] (q11) -- (p11) ;
    \draw[-{Latex[length=3mm]}] (q10) -- (p11) ;
    \draw [] (p10) to[out=320,in=220] (q10);
  \end{tikzpicture}
  \caption{1-round Delayed Lossy-Link}
\end{figure}
\fi

\begin{wrapfigure}{l}{0.35\textwidth}
\vspace{-10pt}
\begin{tikzpicture}[scale=0.9]
	\node[ps] at (0.00, 0.00) (p1r1) { };
	\node[rs] at (1.60, 0.00) (p3r1) { };
	\node[ss] at (2.40, 0.00) (p4r1) { };
	\node[ts] at (3.20, 0.00) (p5r1) { };
	\node[ps] at (0.00, 1.20) (p1r2) { };
	\node[qs] at (0.80, 1.20) (p2r2) { };
	\node[rs] at (1.60, 1.20) (p3r2) { };
	%\node[ss] at (2.40, 1.20) (p4r2) { };
	\node[ts] at (3.20, 1.20) (p5r2) { };
	\node at (1.60, 2.10){ \rotatebox{90}{$\cdots$ }};
	\node[ps] at (0.00, 3.00) (p1r5) { };
	\node[qs] at (0.80, 3.00) (p2r5) { };
	\node[rs] at (1.60, 3.00) (p3r5) { };
	\node[ts] at (3.20, 3.00) (p5r5) { };
	\node[ps] at (0.00, 4.20) (p1r6) { };
	\node[qs] at (0.80, 4.20) (p2r6) { };
	\node[rs] at (1.60, 4.20) (p3r6) { };
	\node[ts] at (3.20, 4.20) (p5r6) { };
	\node[ps] at (0.00, 5.40) (p1r7) { };
	\node[qs] at (0.80, 5.40) (p2r7) { };
	\node[rs] at (1.60, 5.40) (p3r7) { };
	\node[ts] at (3.20, 5.40) (p5r7) { };
	\node[ps] at (0.00, 6.60) (p1r8) { };
	\node[qs] at (0.80, 6.60) (p2r8) { };
	\node[rs] at (1.60, 6.60) (p3r8) { };
	\node[ts] at (3.20, 6.60) (p5r8) { };
	\node at (1.60, 7.50){ \rotatebox{90}{$\cdots$ }};
	\node[ps] at (0.00, 8.40) (p1r11) { };
	\node[qs] at (0.80, 8.40) (p2r11) { };
	\node[rs] at (1.60, 8.40) (p3r11) { };
	\node[ts] at (3.20, 8.40) (p5r11) { };
	\node[ps] at (0.00, 9.60) (p1r12) { };
	\node[qs] at (0.80, 9.60) (p2r12) { };
	\node[rs] at (1.60, 9.60) (p3r12) { };
	\node[ps] at (0.00, 10.80) (p1r13) { };


	%\draw[->] (p5r1) -- (p1r2);
	\draw[->] (p4r1) -- (p1r2);
	\draw[->] (p1r1) -- (p2r2);
	\draw[->] (p1r1) -- (p3r2);
	\draw[->] (p3r1) -- (p5r2);
	\draw[->] (p1r5) -- (p2r6);
	\draw[->] (p2r5) -- (p5r6);
	\draw[->] (p3r6) -- (p1r7);
	\draw[->] (p5r6) -- (p3r7);
	\draw[->] (p2r7) -- (p1r8);
	\draw[->] (p3r7) -- (p1r8);
	\draw[->] (p5r7) -- (p3r8);
	\draw[->] (p3r7) -- (p2r8);
	\draw[->] (p2r7) -- (p3r8);
	\draw[->] (p5r11) -- (p3r12);
	\draw[->] (p2r11) -- (p3r12);
	\draw[->] (p5r11) -- (p2r12);
	\draw[->] (p2r12) -- (p1r13);
	\draw[->] (p3r12) -- (p1r13);
 
    %\draw[->] (-1, 2) -- (-1, 10) node[midway, above left] {$t$};

    \draw[dashed] (-0.8, 4.8) node[left,align=left] {$r_s$} -- (3.7, 4.8) ;

    \node[rectangle,rounded corners,dotted,draw,inner sep=3pt,align=center] at (0, 12.6) (cc1) {\tp};
    \node[rectangle,rounded corners,dotted,draw,inner sep=3pt,align=center] at (1.2, 12.2) (cc2) {\tq \tr};
    \node[rectangle,rounded corners,dotted,draw,inner sep=3pt,align=center] at (2.4, 12.6) (cc3) {\ts};
    \node[rectangle,rounded corners,dotted,draw,inner sep=3pt,align=center] at (3.2, 12.2) (bcc) {\ttt};
    
	%\draw[->] (bcc) -- (cc3);
	\draw (bcc) edge[->,out=230, in=320] (cc2);
	\draw (bcc) edge[->,out=120, in=60]  (cc3);
	\draw (cc2) edge[->,out=140, in=40]  (cc1);

    \draw[dotted,rounded corners] (-0.35,-0.35) rectangle (3.55,4.55);
    \draw[dotted,rounded corners] (-0.35,5) rectangle (0.35,11.5);
    \draw[dotted,rounded corners] (0.45,5) rectangle (1.95,10);
    \draw[dotted,rounded corners] (2.85,5) rectangle (3.55,9);

    \node[align=right] at (-0.8, 13) {$\overline{\G[]}:$};

\end{tikzpicture}
\caption{An example of the causal cone of \tp.
At the top, $\overline{\G[]}$ depicts the integral graph, $r_s$ shows the stabilisation round.}
\label{fig:bounded_causal_cone}
\vspace{-5pt}    
\end{wrapfigure}

%\SetKwData{msgs}{Messages}
%\SetKwData{simState}{state}
%\SetKwData{causalCone}{cc}
%\SetKwData{recipient}{recipient}
%\SetKwData{round}{r}
%\begin{algorithm}
%    \caption{Simulating protocol $\Algo$
%        (defined by $T_{\Algo}, S_{\Algo}$ and the initial configuration $C^0_{\Algo}$)
%        solving a terminating task, in the DLL for process $i$.}
%    \label{alg:minmaxone}
%    \DontPrintSemicolon
%    \SetNoFillComment
%    \SetKwProg{Fn}{def}{:}{}
%    \SetKwFunction{transition}{T}
%    \SetKwFunction{sending}{S}
%    \SetKwFunction{simulate}{simulate}
%    $\simState \gets C^0_{\Algo}(i)$\;
%    $\causalCone = \simState$\;
%    $\round \gets 1$\;
%    \BlankLine
%    \Fn{\transition{\msgs : $\{ \causalCone_{j_1}, \causalCone_{j_2} \dots \}$}}{
%        $\causalCone = \{ i \rightarrow \{ \causalCone_{j_1}, \causalCone_{j_2} \dots \} \}$\;

%        $\round \gets \round + 1$\;
%    }

%    \BlankLine
%    \Fn{\sending{\recipient}}{
%         \KwRet $(i, \causalCone)$ \;
%    }

%    \Fn{\simulate{\causalCone : $\{ m1, m2, \dots \}$}}{
%        $inc_messages \gets \{ \}$\;
%        \For{$m \in \causalCone$}{
%            \If{$m =! $}{
%            
%            }
%        }
        
%        $\simState \gets T_{\Algo}( \simState, \msgs )$\;
%        $S_{\Algo}(\causalCone)$ \;
%    }
%\end{algorithm}


\SetKwData{pAwake}{AwakeProcesses}
\SetKwData{msgs}{Messages}
\SetKwData{round}{r}
\SetKwData{minimum}{currentMin}
\SetKwData{cont}{Contenders}
\begin{algorithm}
    \caption{A protocol to solve stabilising agreement for process $i$.}
    \label{alg:minmaxone}
    \DontPrintSemicolon
    \SetNoFillComment
    \SetKwProg{Fn}{def}{:}{}
    \SetKwFunction{transition}{T}
    \SetKwFunction{sending}{S}
    $\agreementinput \gets v_i$\;
    $\agreementoutput \gets v_i$\;
    $\minimum \gets v_i$\;

    \BlankLine
    \Fn{\transition{\msgs : $\{ \minimum_j, \minimum_l, \dots \}$}}{
        %\tcc{keep the currently received messages}

        $\minimum         \gets \min( \msgs )$\;
        $\agreementoutput \gets \max( \msgs )$\;
    }

    \BlankLine
    \Fn{\sending{ }}{
         \KwRet $\minimum_i$ \;
    }
\end{algorithm}

\iffalse
\section{Any Message Adversary with functionally bounded silence periods is a strongest Message Adversary}

\todo{}
Conversely, the only case where the MinMax algorithms fail by \cref{thm:stabagreeimp},
is when these silence periods grow arbitrarily. Therefore, we conclude that any functionally
bounded message adversary is a strongest message adversary for stabilising agreement.

\begin{theorem}
    Any oblivious DLL message adversary $MA$ with functionally bounded silence periods is a
    strongest Message Adversary.
\end{theorem}

\begin{proof}
    Negating \cref{eq:fun_bounded_ma} results in,
    \begin{equation}\label{eq:unbounded_ma}
        (\forall \Theta : \N \rightarrow \N)\ (\exists \sigma \in MA)\ (\forall R \geq 0)\ 
            (\exists r \geq R)\ \Theta(r) \leq k_{\sigma}(r) = D_{\sigma, \p}(r).
    \end{equation}
    I.e., for any function $\Theta$, there exists a dynamic graph sequence $\sigma$ such that
    its silence bound $k_{\sigma}$ exceeds $\Theta$ infinitely often. Whats left to prove
    is that the existence of such $\sigma$ implies that $MA$ admits unbounded silence
    periods, and thus the inductive definition of the forever undecided sequence in
    \cref{thm:stabagreeimp}.

    As we can choose $\Theta$ freely here, we choose a sequence of functions
    $\Theta_1, \Theta_2, \dots$ such that 
    \[ (\forall i)\ (\forall r)\ \Theta_i(r) < \Theta_{i+1}(r), \]
    and each $\Theta_i$ has corresponding $\sigma$ where $k_{\sigma}$ eventually dominates it.

    As already mentioned, given any $\sigma$, $k_{\sigma}$ is well defined for all $r \in \N$
    and thus every $k_{\sigma}$ is a subset of $\N \times \N$. By \cref{eq:unbounded_ma}, for any
    such $k_{\sigma}$ there exists a $k_{\sigma'}$ that repeatedly eventually dominates it forever,
    i.e., has longer silence periods.
\end{proof}
\fi

\subsection{DLL is equivalent to $\mathcal{AMP}_{2,1}$}

In this section we show that adding the possibility of arbitrary but finite silence periods to the Lossy-Link model intuitively weakens the model to a point where the synchrony properties of the system no longer play a significant role in task solvability.

More precisely, we show that the Delayed Lossy-Link model for two processes is task-equivalent to $\mathcal{AMP}_{2,1}$, the asynchronous crash-resilient message passing model for two processes where at most one process may crash and any message sent will eventually be received. This task equivalence holds for both terminating and stabilising tasks.

\begin{theorem}\label{thm:termAMP}
    Let $T = \langle \mathcal{I}, \mathcal{O}, \Delta \rangle$ be distributed task. $T$ is solvable in the DLL model iff $T$ is solvable in $\mathcal{AMP}_{2,1}$.
\end{theorem}

\begin{proof}
First, assume that $T$ is solvable in the DLL model. It follows from~\cref{thm:TDLLtriv} that $T$ is trivial, and therefore solvable in $\mathcal{AMP}_{2,1}$.

Now assume that $T$ is solvable in $\mathcal{AMP}_{2,1}$ and let $\mathcal{P}$ be a protocol that solves $T$ in $\mathcal{AMP}_{2,1}$. Consider an execution $\sigma_{\tp} \in \mathcal{ASM}_{2,1}$ such that $\tq$ crashes from the start. Since $\mathcal{P}$ solves $T$ then there is a finite amount of steps $k_1$ that $\tp$ takes before deciding $\agreementoutput_{\tp}$. Symmetrically consider an execution $\sigma_{\tq}$ where $\tp$ crashes from the start. It follows that there exists a finite amount of steps $k_2$ that $\tq$ takes before deciding $\agreementoutput_{\tq}$. Now consider an execution $\sigma$ such that $\tp$ and $\tq$ do not crash, and all message reception is deferred by the message scheduler until a time $t_0$ where $\tp$ and $\tq$ have already taken $k =\; _{max} \{ k_1+1, k_2+1\}$ steps. Notice that until time $t_0$, $\sigma$ is indistinguishable from $\sigma_{\tp}$ to $\tp$; and $\sigma$ is also indistinguishable from $\sigma_{\tq}$ to $\tq$. It follows that $\mathcal{P}$ terminates and decides $[\agreementoutput_{\tp}, \agreementoutput_{\tq}]$. Since $\mathcal{P}$ solves $T$, then $[\agreementoutput_{\tp}, \agreementoutput_{\tq}] \in \mathcal{O}$. Note that both $\agreementoutput_{\tp}$ and $\agreementoutput_{\tq}$ were computed without any communication. Therefore $T$ is trivial.
\end{proof}


\textcolor{blue}{This is not a counterexample, since Theorem 6 is about terminating tasks. Furthermore, I am considering that crashed processes that did not crash from the start to have fixed a decision. Namely after crashing, the last decision they made.}

the short term goal is to show that even a single of these crashes is enough to impede stab agreement in the AMP_n,1.

More than one crash is not sane to ask, because if there are more than 2 crashes, then the crashing processes must already have achieved some sort of consensus. 

Yeah, but at time 0, they haven't set a decision. If they crash at time k, they already set a decision. With more than 2 crashes, it is not sensible to consider

usually only non-crashed processes are not requried to do anything.
otherwise the system chrashes processes at time t=0 and requiring them to decide anything, makes the task trivial.

But that is why in no asynchronous system specification i have seen so far any crashed process is required to do anything! Because its impossible with no guarantees on the communication! because messages get delayed until you crash! but then what do you decide?

Yes but no crashing process has to receive anything before it crashes! Requiring crashing processes to do anything requires you to specify that they receive something before crashing! otherwise its a trivial task!

Messages that are sent before crashing will still arrive. 

No, stabilizing protocols make processes decide at each step. Once the process is crashed, 

I can require it for 1 process. If it crashes at start, then no decision has been made, and its ok, but the moment the process makes a step, it already is doomed because it already set a decision. You can indeed require it. There is no limitation that prevents you from requiring it. They are not looking into stab tasks. Crashed processes are not required to do anything.
It is the live processes that are forced to agree with the single crashed process. Yes, I am not using it, I do not need to know whether a process crashed or not. For example, lets say your last decision was to decide on a number 2. afterwards you died. I have no idea that you died. Still I must decide on something that agrees with your last will. It is exactly the same as the DLL.

I cannot solve stab consensus on it, but I can solve stab approximate agreement.

What? Theorem 6 equates tasks between DLL in SMP and no FD in AMP. This implies, that i can solve anything on DLL in SMP that can be solved in AMP with no failure detector. Algorithm2 provides a way to solve stabag im AMP. Therefore i can solve it in DLL SMP.

OK, i see your point.




I stand by my point here, this does not work.

It does. Bear with me. Single process is allowed to crash, just one. However, if such process at some point sets a decision \delta(r), and then crashes immediately after, then this \delta(r) is its final will. It will not be changed because it died. The rest of the processes have absolutely no way of knowing that it crashed.  Yes, and how do the others now also decide \delta(r)? The same way they would decide if the crashed process was just arbitrarily silent

x_p, and x_q are inputs. x_p wins over x_q. After one message q -> p i delay any further message q -> p. At any time p cannot distinguish this run from a run where q is still alive, and thus has heard of p's value, also deciding x_p, from a run where q already died, and, to p's best knowledge, x_q is q's last wish! what does p do? p decides on x_p? that is wrong in the run where q is alive, as q does not know x_p. p decides on x_q? but then this is indistinquishable for p from the run where q receives x_p and decides x_p because it wins over x_q! this is already assuming how the protocol works! yes sure, but i can have assumptions about decisions using indistinguishability arguments. at no point in any prefix i am delivering anything to q! Exactly, this is the same proof as the DLL impossibility.

Yeah, but this is exactly the point in the DLL indistinguishability arguments. There is no way of defining the decisions in a correct way, because they might be final or they might be temporary from the silence.
Yes, but i don't understand what you are trying to tell me, clearly you cannot require a task to respect crashed decisions without any further communication restrictions.

Theorem 6 is about Terminating tasks. I don't need to simulate anything. Theorem 6 shows that the only terminating tasks in AMP 2,1 are trivial tasks
the same as the terminating tasks in the DLL

This is impossible in the classical definition of asynchronous systems with crashes.

Sure you can require it, but i will provide you a counterexample for anything you specifiy on an asynchronous system where crashed processes are required to do anything. Either you make the requirement loose enough, or its impossible. Loose enough = trivial task. That is literally the core of the proof of FLP, you cannot know whether a process crashed or not.

-> Yes, but that decision is not required to agree with other, correct, i.e., non-crashed processes by the task definition. Raynald & Stainer also took that route, just excusing crashed processes.

\textbf{Counterexample}: stabilising agreement is solvable in $\mathcal{A}_{n,n-1}$.
By \cref{thm:termAMP} this implies (by the iff direction) that there exists an algorithm
solving stabilising agreement in the DLL (by simulating \cref{async:stabag} on
$\mathcal{A}_{n,n-1}$), directly contradicting \cref{thm:stabagreeimp}.

\SetKwData{msgs}{Messages}
\SetKwData{simR}{simRound}
\SetKwData{simstate}{simState}
\SetKwData{inits}{initialStates}
\begin{algorithm}
    \label{async:stabag}
    \caption{Algorithm solving stabilising agreemnt in $\mathcal{A}_{n,n-1}$, code for process $p$.}
    \DontPrintSemicolon
    \SetNoFillComment
    \SetKwProg{Fn}{def}{:}{}
    \SetKwFunction{transition}{T} \SetKwFunction{sending}{S}
    $\agreementoutput \gets \agreementinput$\;
    \BlankLine
    \Fn{\transition{\msgs : $\{ \agreementoutput_{q_1}, \agreementoutput_{q_2}, \dots \}$}}{
        $\agreementoutput \gets \min(\msgs)$\;
    }
    \BlankLine
    \Fn{\sending{ }}{
         \Return $\agreementoutput$ \;
    }
\end{algorithm}

\begin{proof}
    By definition all correct, i.e., non-crashed, processes have to eventually agree. As
    every \emph{correct} $p$ process hears from all other correct processes, it will in line 3,
    hear from the minimum input value among the correct processes. As all other correct processes
    also eventually hear from the correct process $p$, they will also stablisie on the lowest
    value $p$ has heard of.
\end{proof}

Now that we have established the equivalence between terminating tasks in the DLL model, and terminating tasks in $\mathcal{AMP}_{2.1}$ we will extend this equivalence to stabilising tasks. We show this equivalence by translating an individual process history in the DLL model, $\mathcal{H}$, to a corresponding history $\mathcal{H}'$ in $\mathcal{AMP}_{2,1}$ and viceversa. These translations enable us to simulate a stabilising protocol for $\mathcal{AMP}_{2,1}$ in a $DLL$ execution and respectively a stabilising protocol for DLL in $\mathcal{AMP}_{2,1}$.

\emph{----------OLD PROOF---- DO NOT DELETE YET-------------}

%%%%%%%%%%%%%%%%%%% OLD PROOF %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    Assume for a contradiction that $T$ is solvable as a stabilising task in the Delayed Lossy-Link model, but not as a terminating task in the Lossy-Link model. We will proceed in the same fashion as in \cref{thm:stabagreeimp} in order to build an execution that does not stabilize.

    Let $\mathcal{P}$ be a protocol that solves $T$ as a stabilising task in the DLL model. Consider the communication patterns $\sigma_{(1,1)} = \tqp \comp \tpq^{\omega}; \; \sigma_{(1,2)} = \tpqp \comp \tpq^{\omega}; \;\sigma_{(1,3)} = \tpq^{\omega}; \; \sigma_{(2,1)} = \tqp^{\omega}; \; \sigma_{(2,2)} = \tpqp \comp \tqp^{\omega}; \;\sigma_{(2,3)} = \tpq \comp \tqp^{\omega}$. Let $S_0$ be the set of input configurations $\config[0]$, such that either $\mu_1 = [\decfinalp{\config[0]\comp \sigma_{(1,1)}}{\tp}, \decfinalp{\config[0]\comp \sigma_{(2,1)}}{\tq}], \mu_2 = [\decfinalp{\config[0]\comp \sigma_{(1,2)}}{\tp}, \decfinalp{\config[0]\comp \sigma_{(2,2)}}{\tq}]$, or \\
    $\mu_3 = [\decfinalp{\config[0]\comp \sigma_{(1,3)}}{\tp}, \decfinalp{\config[0]\comp \sigma_{(2,3)}}{\tq}]$ are invalid output configurations. $S_0 \neq \varnothing$, otherwise for each initial configuration $\config[0]$, $\mu_1$, $\mu_2$, and $\mu_3$ are valid output configurations. Notice that $\decfinalp{\config[0] \comp \sigma_{(1,1)}} {\tp}$, $ \decfinalp{\config[0]\comp\sigma_{(1,2)}} {\tp},$ and $\decfinalp{\config[0]\comp\sigma_{(1,3)}} {\tp}$ are computable at $\config[0]\comp\tqp, \config[0] \comp \tpqp,$ and $\config[0] \comp \tpq$ respectively, since $\tp$ does not receive any further information throughout the rest of the executions $\sigma_{(1,1)}, \sigma_{(1,2)},$ and $\sigma_{(1,3)}$. Symmetrically, $\decfinalp{\config[0]\comp\sigma_{(2,1)}} {\tq}, \decfinalp{\config[0]\comp\sigma_{(2,2)}} {\tq},$ and $\decfinalp{\config[0]\comp\sigma_{(2,3)}} {\tq}$ are computable at $\config[0]\comp\tqp, \config[0] \comp \tpqp,$ and $\config[0] \comp \tpq$ respectively. Consider the following 1-round protocol $\mathcal{P}'$ where if $\tp$ receives a message, then it decides $\decfinalp{\config[0]\comp \sigma_{(1,1)}}{\tp}$, else it decides $\decfinalp{\config[0]\comp \sigma_{(1,3)}}{\tp}$. Reciprocally, if $\tq$ receives a message, then it decides $\decfinalp{\config[0]\comp \sigma_{(2,3)}}{\tq}$, else it decides $\decfinalp{\config[0]\comp \sigma_{(2,1)}}{\tq}$. Notice that if the adversary plays $\config[0] \comp \tqp$, then $\mathcal{P}'$ will decide $[\decfinalp{\config[0]\comp \sigma_{(1,1)}}{\tp}, \decfinalp{ \config[0] \comp \sigma_{(2,1)}}{\tq}] = \mu_1$ which is a valid output configuration. Reciprocally if the adversary plays $\config[0]\comp\tqp$, then $\mathcal{P}'$ will decide $[\decfinalp{\config[0]\comp \sigma_{(1,3)}}{\tp}, \decfinalp{ \config[0] \comp \sigma_{(2,3)}}{\tq}] = \mu_3$, which is also a valid output configuration. Since $\sigma_{(1,1)}$ is indistinguishable from $\sigma_{(1,2)}$ to $\tp$, and $\sigma_{(2,3)}$ is indistinguishable from $\sigma_{(2,2)}$ to $\tq$; it follows that $\decfinalp{\config[0]\comp \sigma_{(1,1)}}{\tp}= \decfinalp{\config[0]\comp \sigma_{(1,2)}}{\tp}$, and $\decfinalp{\config[0]\comp \sigma_{(2,3)}}{\tq}= \decfinalp{\config[0]\comp \sigma_{(2,2)}}{\tq}$. Finally, if the adversary plays $\config[0]\comp \tpqp$ then $\mathcal{P}'$ decides $[\decfinalp{\config[0]\comp \sigma_{(1,1)}}{\tp}, \decfinalp{\config[0]\comp \sigma_{(2,3)}}{\tq} ] = [\decfinalp{\config[0]\comp \sigma_{(1,2)}}{\tp}, \decfinalp{\config[0]\comp \sigma_{(2,2)}}{\tq} ] = \mu_2$, which is a valid output configuration. This contradicts that $T$ cannot terminate in the Lossy Link model, and therefore either $\mu_1$, $\mu_2$ or $\mu_3$ are invalid output configurations. 
    
    As in the proof of \cref{thm:stabagreeimp}, there exists an $r_1 \in \N$ such that $[\delta_{\tp}(\config[0]\comp\tqp \comp \tnone^{r_1}), \delta_{\tq}(\config[0]\comp \tqp \comp \tnone^{r_1})] = \mu_1$, $[\delta_{\tp}(\config[0] \comp \tpqp \comp \tnone^{r_1}), \delta_{\tq}(\config[0]\tpqp \comp \tnone^{r_1})] = \mu_2$, and $[\delta_{\tp}(\config[0]\comp\tpq \comp \tnone^{r_1}), \delta_{\tq}(\config[0]\comp\tpq \comp \tnone^{r_1})] = \mu_3$.

    Let $S_1$ be the set of prefixes $\config[0]\comp G \comp \tnone^{r_1}$ such that $G \in \{\tqp, \tpqp, \tpq\}$ that yield invalid output configurations, and that extend the set of initial configurations $S_0$.

    We can inductively repeat this procedure to obtain sets of prefixes $S_{i+1} \neq \varnothing$ such that each prefix $P \in S_{i+1}$ is an extension of a prefix $P' \in S_{i}$, and $\delta(P)$ is an invalid output configuration.

    Applying König's Lemma to the prefix sets $S_{i}$, allows us to find an infinite graph sequence $\sigma_{\infty}$ that infinitely often reaches invalid output configurations. This contradicts that $\mathcal{P}$ solves a $T$ as a stabilising task in the Delayed Lossy-Link model.

    %We construct a simulator based on the very simple idea that any Lossy-Link admissible
    %sequence is either equal to $\tpqp^{\omega}$ or there is one process which does not
    %receive the other process' message first.
%%%%%%%%%%%%%%%%%%% OLD PROOF %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    \iffalse
    Consider the following extensions to $\pi$, where each $\sigma_{(1, j)}$ 
    \[ \sigma_{(1,1)}=\pi \comp \tqp  \comp \tpq^{\omega},
       \sigma_{(1,2)}=\pi \comp \tpqp \comp \tpq^{\omega}, 
       \sigma_{(1,3)}=\pi \comp \tpq  \comp \tpq^{\omega}. \]
    Symmetrically consider the following communication patterns
    \[ \sigma_{(2,1)}=\pi \comp \tqp  \comp \tqp^{\omega},
       \sigma_{(2,2)}=\pi \comp \tpqp \comp \tqp^{\omega},
       \sigma_{(2,3)}=\pi \comp \tpq  \comp \tqp^{\omega}. \]
    Notice that all of these communication patterns are admissible under the DLL model. Since
    we assume that $\mathcal{P}$ solves stabilising agreement, $\mathcal{P}$ stabilizes on a
    decision value.
    
    Notice that $\decfinal{\sigma_{(1,3)}} \neq \decfinal{\sigma_{(2,1)}}$ as $\tp$ never received
    a message from $\tq$ at $\decfinal{\sigma_{(1,3)}}$, and reciprocally $\tq$ never received a
    message from $\tp$ at $\decfinal{\sigma_{(2,1)}}$.
    Now consider
    \[ r^* = max\{ \stabround{\mathcal{P}}{\sigma_{(i,j)}}\ |\ i \in \{1,2\}, \; j\in \{1,2,3\} \}.\]

    Notice that the $r^*$ prefix of $\sigma_{(1,1)}$, i.e., $\tqp \comp \tpq^{r^*-1}$ is
    indistinguishable from $\tqp \comp \tnone^{r^*-1}$ for $\tp$.
    implying that $\tp$ has a decision value of $\decfinal{\sigma_{(1,1)}}$ at round $r^*+1$
    with prefix $\tqp \comp \tnone^{r^*}$.
    
    Symmetrically $\tp$ decides $ \decfinal{\sigma_{(1,2)}}$, and $\decfinal{\sigma_{(1,3)}}$ for
    $\tpqp \comp \tnone^{r^*}$ and $\tqp \comp \tnone^{r^*}$ respectively.

    In an analogous way, notice that $\tq$ decides $\decfinal{\sigma_{(2,1)}}$ for $\tqp \comp \tnone^{r^*-1}$, $\decfinal{\sigma_{(2,2)}}$ for $\tpqp \comp \tnone^{r^*}$, and $\decfinal{\sigma_{(2,3)}}$ for $\tpq \comp \tnone^{r^*}$.

    We assert that $\mathcal{P}$ has conflicting decisions at either $\tqp \comp \tnone^{r^*}$, $\tpqp \comp \tnone^{r^*}$, or $\tpq \comp \tnone^{r^*}$. 

    \begin{tikzpicture}
        \node at (.5,  0) (r1) {$\delta_{\tp}(\pi_k )$};
        \node at (0, -1) (r2) {$\delta_{\tp}(\pi_k : \tpq   : \tnone^r)$};
        \node at (0, -2) (r3) {$\delta_{\tq}(\pi_k : \tpq   : \tnone^r)$};
        \node at (0, -3) (r4) {$\delta_{\tq}(\pi_k : \tpqp  : \tnone^r)$};
        \node at (0, -4) (r5) {$\delta_{\tp}(\pi_k : \tpqp  : \tnone^r)$};
        \node at (0, -5) (r6) {$\delta_{\tp}(\pi_k : \tqp   : \tnone^r)$};
        \node at (0, -6) (r7) {$\delta_{\tq}(\pi_k : \tqp   : \tnone^r)$};
        \node at (.5, -7) (r8) {$\delta_{\tq}(\pi_k )$};
    
        \foreach \i in {1, 3, 5, 7} {
            \pgfmathtruncatemacro{\j}{\i+1}
            \draw (r\i.west) .. controls +(left:0.4cm) and +(left:0.4cm) .. (r\j.west)
                node[midway,draw,circle,inner sep=2pt,fill=white] (edge{\i}{\j}eq) {$=$};
        }
    
        \foreach \i in {2, 4, 6} {
            \pgfmathtruncatemacro{\j}{\i+1}
            %\draw (r\i.south) .. controls +(right:2cm) and +(right:2cm) .. (r\j.south)
            \draw (r\i.east) .. controls +(right:0.4cm) and +(right:0.4cm) .. (r\j.east)
                node[midway,draw,circle,inner sep=2pt,fill=white] (edge{\i}{\j}id) {id};
        }
    
        \draw (r1.east) .. controls +(right:2cm) and +(right:2cm) .. (r8.east)
            node[midway,draw,circle,inner sep=2pt,fill=white] (edgeneq) {$\neq$};

        \iffalse
        \node[align=center,rectangle,rounded corners,draw] at (5, 6) (ex1)
            {$\agreementoutput_{\tp}(\sigma : \tnone : \tnone^k)$ and\\
             $\agreementoutput_{\tq}(\sigma : \tnone : \tnone^k)$\\
             are not equal as\\
             $\sigma$ is stably undecided\\
             by assumption};
        \draw[->,dotted] (ex1.south) .. controls +(south:1cm) and +(east:1cm) .. (edgeneq.east);
    
        \node[align=center,rectangle,rounded corners,draw] at (-4.5, 4) (ex2)
            {$\agreementoutput_{\tp}$, $\agreementoutput_{\tq}$ are equal\\
                as the prefixes are\\
                indistinguishable};
        \foreach \i in {1, 3, 5, 7} {
            \pgfmathtruncatemacro{\j}{\i+1}
            \draw[->,dotted] (ex2.east) .. controls +(east:1cm) and +(west:1cm) ..
                (edge{\i}{\j}eq.west);
        }
        
        \node[align=center,rectangle,rounded corners,draw] at (5, 1.5) (ex3)
            {Identical runs};
        \foreach \i in {2, 4, 6} {
            \pgfmathtruncatemacro{\j}{\i+1}
            \draw[->,dotted] (ex3.west) .. controls +(west:2.4cm) and +(east:1cm) ..
                (edge{\i}{\j}id.east);
        }
        \fi
    \end{tikzpicture}
    \fi


    \iffalse
For any non-empty kernel sequence $\G(r)$ we can at any round $r$ define the number of rounds
it took a process of the kernel to reach all other processes. We denote by $D_{\sigma, \p}(r)$ the
smallest number of rounds it took $\p$ to reach everybody else by round $r$, formally
\[ D_{\sigma, \p}(r) = \min\{ k\ |\ (\forall \q \in \Pi)\ \p \pq \q \in \G(r-k : r) \} . \]
By convention, if $\p$ never reaches some other process, then this set is empty and
so $D_{\sigma, \p}(r) = \infty$.

\begin{corollary}
    For any perpetual broadcaster $\p \in Ker(\sigma)$, $D_{\p}(r)$ is finite for every
    round $r$, formally
    \[ (\forall \p \in Ker(\sigma))\ (\forall r)\ D_{\sigma, \p}(r) < \infty . \]
\end{corollary}

The previously introduced MinMax algorithm solve stabilising agreement
under a message adversary $MA$ if (and not only if) the information decimination from 
the kernel to all other processes is bounded by some $k_{\sigma}$ for every dynamic
graph sequence $\sigma \in MA$
\[ (\forall \p \in Ker(\sigma))\ (\forall r)\ D_{\sigma, \p}(r) < k_{\sigma} . \]
In this case, we can also define $k_{\sigma}$ explicitly, given a run $\sigma$
\[ k_{\sigma} = \max \{ D_{\sigma, \p}(r)\ |\ \forall r, \forall \p \in Ker(\sigma) \} , \]
one can verify that this implies the above equation.
%\[ |S^0| < k_{\sigma}, |S^1| < k_{\sigma}, \dots. \]
As already argued, some monotonically increasing diameter guesser $\Theta(r)$ will eventually
surpass any such fixed $k_{\sigma}$ in every graph sequence in $MA$. In other words,
there exists a silence guesser function $\Theta$ that eventually surpasses $k_{\sigma}$ for
every $\sigma \in MA$:
\begin{equation}
    (\exists \Theta : \N \rightarrow \N)\ (\forall \sigma \in MA)\ (\exists R \geq 0)\ 
       (\forall r \geq R)\ \Theta(r) > k_{\sigma},
\end{equation}
implying that any message adversary with bounded dynamic graph sequences admits solving stabilising
agreement.

We extend this from fixed bound per dynamic graph sequence to any functional silence bound
$k_{\sigma}(r)$ per sequence, defined by
\[ k_{\sigma}(r) = \max \{ D_{\sigma, \p}(r)\ |\ \forall \p \in Ker(\sigma) \} , \]
Note that $k_{\sigma}(r)$ is well defined for every $r$, as we require a non-empty kernel
and thus some communication eventually happens making every $D_{\sigma, \p}$ finite.
With this we tie solve-ability of stabilising agreement using a MinMax algorithm to the
existence of a function that eventually dominates every functional silence bound
$k_{\sigma}(r)$ for every $\sigma \in MA$:
\begin{equation} \label{eq:fun_bounded_ma}
    (\exists \Theta : \N \rightarrow \N)\ (\forall \sigma \in MA)\ (\exists R \geq 0)\ 
        (\forall r \geq R)\ \Theta(r) > k_{\sigma}(r).
\end{equation}
\fi

% \section{Stabilising agreement in the Lossy-Link Model}

% %The IIS corresponds to the tournament message adversary with the additional restriction
% %that every round graph is equivalent to its transitive closure. This implies a bounded 
% Any round graph in the lossy-link model has a bounded rootedness of $T=1$ in the sense of
% \cite[Definition 4]{CM19:DC} and therefore we can directly employ a MinMax algorithm with
% a known bound of $1$. Rootedness denotes the maximum number of edges in the shortest path
% between any two processes. Any lossy link graph is trivially rooted.

% \begin{theorem}\label{thm:llroot}
%     The \emph{Lossy-Link} adversary has a \emph{rootedness} of $T=1$, meaning every round-graph
%     $\G(r)$ contains at least one process that directly reaches everybody else:
%     \[ \forall r : \exists \p : \forall \q : \p \pq \q \in \G(r).\]
% \end{theorem}

% \begin{proof}
%     By a case analysis on the set of possible round graphs $\{ \tpq, \tpqp, \tqp \}$, where
%     each of them has one process reaching all other processes via a direct edge.
% \end{proof}

% \iffalse
% \begin{proof}
%     We build a chain of increasing sets of processes, $U_{\p} \subset U^1_{\q_1} \dots U^k_{\q_k}$,
%     where each set corresponds to the outgoing neighbors of one process 
%     $U_{\p} = \{ \q\ |\ \p \pq \q \}$.
%     As $\Pi$ is finite, the last set $U^k_{\q_k}$ is the set of all processes $\Pi$.
    
%     Pick any process $\p$, if $U_{\p} = \Pi$, then $\p$ reaches all other processes in
%     one step already. So lets assume $U_{\p} \neq \Pi$.

%     Then there exists some $\q$ where $\p \not\pq \q$ and therefore
%     $\p \qp \q$ and by transitivity $\q \rightarrow \q'$ for every $\q'$ where $\p \pq \q'$. 
%     This implies any outgoing neighbor of $\p$ is also an outgoing neighbor of $\q$ and additionally
%     $\p$ is an outgoing neighbor of $\q$, so $U_{\p} \subset U_{\q}$ holds.
    
%     Now either $U_{\q} = \Pi$ and we have found one process that reaches all other processes
%     in one step, or $U_{\q} \neq \Pi$ and we can apply our induction step again.
% \end{proof}
% \fi

% This proves that stabilising agreement is solvable in the non-delayed lossy-link model. This
% stands in sharp contrast to the following section, where arbitrary delays imply impossibility.

\iffalse
\begin{proof}
    We build a chain of increasing sets of processes, $U_{\p} \subset U^1_{\q_1} \dots U^k_{\q_k}$,
    where each set corresponds to the outgoing neighbors of one process 
    $U_{\p} = \{ \q\ |\ \p \pq \q \}$.
    As $\Pi$ is finite, the last set $U^k_{\q_k}$ is the set of all processes $\Pi$.
    
    Pick any process $\p$, if $U_{\p} = \Pi$, then $\p$ reaches all other processes in
    one step already. So lets assume $U_{\p} \neq \Pi$.

    Then there exists some $\q$ where $\p \not\pq \q$ and therefore
    $\p \qp \q$ and by transitivity $\q \rightarrow \q'$ for every $\q'$ where $\p \pq \q'$. 
    This implies any outgoing neighbor of $\p$ is also an outgoing neighbor of $\q$ and additionally
    $\p$ is an outgoing neighbor of $\q$, so $U_{\p} \subset U_{\q}$ holds.
    
    Now either $U_{\q} = \Pi$ and we have found one process that reaches all other processes
    in one step, or $U_{\q} \neq \Pi$ and we can apply our induction step again.
\end{proof}
\fi

\iffalse
$\view^r_{\p}(0)$ contains an edge for every message received in this round, $\view^r_{\p}(-1)$ contains
edges for all messages received last round, directly or indirectly, and so on. Formally, we define a view via
a given graph sequence in \cref{eq:view}, an example procedure implementing it is given in \cref{proc:update}.

\begin{equation}\label{eq:view}
    \G:\view^r_{\p} = \begin{cases}
        \hfill 0 &: \{ \p \qp \q\ |\ \q \in \In^{a}_{\p}(\G(r)) \} \\
        \hfill\vdots& \\
        \hfill-k &: \bigcup\limits_{\q \in V(\view^r_{\p}(-k+1))} 
                    \{ \q \qp \q'\ |\ \q' \in \In^{a}_{\q}(\G(r-k)) \} \\
    \end{cases}
\end{equation}

Note that $\view_{\p}(r)$ is always a subset of the actual graph sequence $\G$ of the run
(modulo a shift of the indices, depending on the round $\p$ woke up).
Further note that, after $\p$ received a message from $\q$, $\p$ is certain about the arrival
(or non-arrival) of all previous messages from $\p$ to $\q$ and thus is certain about those
edges in the actual graph sequence $\G$. In addition to that, $\p$ acquires knowledge about $\q$'s view in
the round where $\p$ received a message from $\q$, denoted as $\view^r_{\p}|_{\q}$ and defined as
\[ \view^r_{\p}|_{\q} = \view^{r'}_{\q}
    \text{ where } r' = \max\bigl\{ 0 < k \leq r\ |\ \p \qp \q \in \G(k) \bigr\}-1. \]
This implies that $\view^r_{\p}|_{\p}$ maps to the view $\p$ had one round earlier, i.e., 
$\view^r_{\p}|_{\p} = \view^{r-1}_{\p}$. Similarly, $\view^r_{\tp}|^{d}$ restricts the view to the view
$\p$ had $d$ rounds ago and shifts the indices accordingly, i.e., $\view^r_{\tp}|^{d}(k) = \view^r_{\tp}(k-d)$.
Finally, we define the length of a view $|\view^r_{\tp}|$
as the (positive) amount of non-empty graphs in it, i.e.,
$|\view^r_{\tp}| = |\{ k \in \Z\setminus\N\ |\ \view^r_{\tp}(k) \neq \emptyset \}|$.
Note that this works because every round all processes send a message to themselves which cannot
be suppressed. Thus every round where $\p$ is awake contains at least one edge (namely the self-loop).
The length of a view can be longer than the process is awake, which is the case when $\p$ hears from
a process that has been awake longer.

We say the view of process $\p$ is \emph{certain} up to round $R$, if $\p$ can fully reconstruct the
active communication graph sequence $\G^a$ up to round $R$. This is possible if, and only if, $\p$
knows what all other processes have received up to round $R$, i.e., 
$(\forall \q \in \Pi)\ \p \qp \q \in \G^a(R:r)$, implying that
$(\forall k \leq R)\ \view^r_{\p}(-k-(r-R)) = \G^a(R-k)$
holds, i.e., starting from $(r-R)$ ago (the number of rounds it took all other processes to reach $\p$),
$\p$'s view matches the graph sequence down to the first round where a process woke up.
\fi

\iffalse
\begin{theorem} \label{thm:BAMPtoLL}
    Let $\Prot$ be a protocol that solves consensus in the $\LL$. Then there exists a protocol $\Prot'$ that solves stabilizing agreement in the $\BAMP_{2,0}$.
\end{theorem}

\begin{proof}
    We present ~\cref{alg:BAMPtoDLL} that maps asynchronous view from the $\BAMP_{2,0}$ model into a corresponding simulated synchronous view in the $\LL$ message adversary. Intuitively, each processes numbers each of their asynchronous steps, and treats them as synchronous rounds. For instance, if process $\tp$ has received  a message from $\tq$ that includes the state of $\tq$ at step $r-1$ before $\tp$ starts its step $r$, then we simulate that $\tp$ received a message from $\tq$ at round $r$. 

    \todo{should be a procedure}
    \SetKwData{msgs}{Messages}
    \SetKwData{simR}{simRound}
    \SetKwData{simstate}{simState}
    \SetKwData{inits}{initialStates}
    \SetKwData{st}{step}
    \SetKwData{sview}{syncView}
    \begin{algorithm}
        \caption{Algorithm that simulates a \DLL stabilizing protocol in the $\BAMP_{2,0}$ model.
        The pseudocode assumes the running process has id $\protect\tp$.}\label{alg:BAMPtoDLL}
        \DontPrintSemicolon
        \SetNoFillComment
        \SetKwProg{Fn}{def}{:}{}
        \SetKwFunction{transition}{T}
        \SetKwFunction{sending}{S}
        $\st_{\tp} \gets 0$\;
        $(\sview_{\tp}, \inits) \gets (\emptyset, \textbf{input})$\;
        $\simstate  \gets \textbf{sim}_{\Prot}(\view_{\tp}, \inits)$\;
        \BlankLine
        \Fn{\transition{\msgs : $\{ (\sview_{\tp}, \inits, \st_{\tp}), \dots \}$}}{
            $\st_{\tp} \gets \st_{\tp}+1$\;
            \If{$\sview_{\tp}[\st_{\tp}] = \emptyset$}{
                $\sview_{\tp}[\st_{\tp}] \gets \tnone$\;
            }
            \ForEach{$(\sview_{\tq}, \inits, \st_{\tq}) \in \msgs$}{
                $(\sview_{\tp}, \inits) \gets (\sview_{\tp}, \inits) \cup (\sview_{\tq}, \inits)$\;
                $\sview_{\tp}[\st_{\tq}]  \gets \tqp$\;
            }
            $\simstate \gets \textbf{sim}_{\Prot}(rmv(\sview_{\tp}),  \inits)$\;
        }
        \BlankLine
        \Fn{\sending{ }}{
             \Return $(\sview_{\tp}, \inits, \st_{\tp})$ \;
        }
    \end{algorithm}
    
    \SetKwData{msgs}{Messages}
    \SetKwData{simR}{simRound}
    \SetKwData{simstate}{simState}
    \SetKwData{inits}{initialStates}
    \SetKwData{phist}{partialHistoryVector}
    \begin{procedure}
        \caption{sim{\DLL}in{\BAMP}($\protect\view_{\protect\tp}$)}
        \label{proc:simadv}
        \SetAlgoRefName{sim\Adv}
        \DontPrintSemicolon
        \SetNoFillComment
        $\phist(\tp) \gets \view_{\tp}$\;
        \If{\p = leader\_id}{
            \ForEach{$\p \in \Pi(\Adv) \setminus \{ \tp, \tq \}$}{
                $\view_{\p} \gets \emptyset$\;
                \ForEach{$0 \geq r > -|\view_{\tp}|$}{
                    $\view_{\p}(r) \gets ( \p \leftarrow \tp )$\;
                }
                $\phist(\p) \gets \view_{\p}$\;
            }
        }
        \Return $\phist$\;
    \end{procedure}

Assume the simulated graph sequence $\G$ inducing $\sview_{\tp}$ and $\sview_{\tq}$ is not an admissible
Delayed Lossy Link sequence, i.e., it has an infinite silent suffix. This implies that neither $\tp$,
nor $\tq$ add an edge to $\sview$, implying that neither receive another message contradicting
broadcast liveness of $\BAMP_{2,0}$.

Since $\Prot$ is a terminating protocol in the \LL and $\h(r)$ is the wait-free core of $\G(r)$, then there exists a
termination round $k$ at $\h(r)$. This means that $\Prot$ terminates with the finite prefix $\h(1,k)$. Since $\h(r)$
is the wait-free core of $\G(r)$, there exists a $k'\geq k$ such that $\h(1,k)$ is the wait-free core of $\G(1,k')$.
Let $t_{\tp}= \max\{ \sigma_{\rho}(\tp, \rho_{\tp}(i).\text{time})< \infty \; \vert \; 0 \leq i \leq k' \}$.
Reciprocally $t_{\tq} =\;  \max\{ \sigma_{\rho}(\tq, \rho_{\tq}(i).\text{time})< \infty \; \vert \; 0 \leq i \leq k'  \}$.
Now let $t_{max} = \; _{\text{max}} \{ t_{\tp}, t_{\tq}\} $. From the definition of $t_{max}$, all of the messages
sent up to step $k$ have already been either delivered or dropped. It follows that after time $t_{max}$,
~\cref{alg:BAMPtoDLL} will always estimate the wait-free core of finite prefix $\G(1,k')$, $\h(1,k)$.
Since $\h(1,k)$ is a terminating prefix for $\Prot$, it follows that ~\cref{alg:BAMPtoDLL} stabilizes at time
$t_{max}$. Since we assume that $\BAMP_{2,0}$ is free from Zeno behavior, there exists a finite step $s_f$
that happens after $t_{max}$ for both $\tp$ and $\tq$. Finally, this shows that ~\cref{alg:BAMPtoDLL}
stabilizes at both step $s_f$ and at time $t_{max}$.

\end{proof}
\fi

\iffalse
\iffalse
Further we also define the notion of \emph{weak $f$-crash-resilient} tasks, denoting a task that can tolerate $f$ arbitrary crashes.
\begin{definition}[Weak Crash-resilient Task/Stabilizing Task] \label{def:crashtask}
    We say that a stabilizing task $\langle \mathcal{I}, \mathcal{O}, \stabtask \rangle$ is $f$-crash resilient if for any input configuration $I_S$ with a set $S$ of correct processes such that $O_S \in \stabtask(I_S)$, then for any subset $S' \subset S$ such that $\vert S' \vert \geq n-f$, $O_{S'} \in \stabtask(I_{S'})$.
\end{definition}
\fi

\begin{definition}[Weak scaling Task/Stabilizing Task] \label{def:scaletask}
    We say that a (stabilizing) task $T_{\Adv} = \langle\mathcal{I}, \mathcal{O}, \task\rangle$ is weak scaling if and only if there exists an adversarial model \Bdv and a task $T_{\Bdv}$ where $\Pi(\Adv) \subset \Pi(\Bdv)$ and 
    \[ (\forall v \in I(T_{\Adv}),\ \exists v' \in I(T_{\Bdv}))\ v = \pi(v') \wedge
        T_{\Adv}(\task)(v) = \pi(T_{\Bdv}(\task)(v')). \]
\end{definition}

The 'dual' of theorem \cref{def:scaletask} defines when a task can be solved even though only a subset of processes are still correct, i.e., non-crashed. We call such tasks \emph{weakly crash-resilient}.

\begin{definition}[Weak crash-resilient Task/Stabilizing Task] \label{def:crashtask}
    We say that a (stabilizing) task $T_{\Adv} = \langle\mathcal{I}, \mathcal{O}, \task\rangle$ is weak crash-resilient if and only if there exists an adversarial model \Bdv and a task $T_{\Bdv}$ where $\Pi(\Bdv) \subset \Pi(\Adv)$ and 
    \[ (\forall v \in I(T_{\Adv}),\ \exists v' \in I(T_{\Bdv}))\ \pi(v) = v' \wedge
        \pi(T_{\Adv}(\task)(v)) = T_{\Bdv}(\task)(v'). \]
\end{definition}
\todo{define $\pi$ as the projection onto process indices}

Note, for example, that any agreement task can be seen as weakly crash-resilient.
\fi

\iffalse
\begin{figure}[ht]
    \centering
    \begin{tikzcd}
        \model_{\Adv \times I_{\Adv}}
            \arrow[r, hook, "\simul"]
            \arrow[d, "\task_{\Adv}"] 
        & \model_{\Bdv \times I_{\Bdv}}
            \arrow[d, "\Prot_{\Bdv}"] \\
        O_{\Adv} & O_{\Bdv}
            \arrow[l, "\pi_{\Adv}"]
    \end{tikzcd}
    \begin{tikzcd}
        \model_{\Adv \times I_{\Adv}}
            \arrow[r, hook, "\simul"]
        & \model_{\Bdv \times I_{\Bdv}}
    \end{tikzcd}
    \caption{A diagram showing the relations a simulation has to satisfy. Usually we will omit the second row with $O_{\Adv}$ and $O_{\Bdv}$. The model $\model_{\Adv \times I_{\Adv}}$ is a simbeddable of $\model_{\Bdv \times I_{\Adv}}$ if, and only if, $\task_{\Adv}= \pi \circ \task_{\Bdv} \circ \simul$, i.e., \Bdv can be used to solve the task }
\end{figure}
\fi

